Towards Transferring Tactile-based Continuous Force Control Policies from Simulation to Robot

The advent of tactile sensors in robotics has sparked many ideas on how robots can leverage direct contact measurements of their environment interactions to improve manipulation tasks. An important line of research in this regard is that of grasp force control, which aims to manipulate objects safely by limiting the amount of force exerted on the object. While prior works have either hand-modeled their force controllers, employed model-based approaches, or have not shown sim-to-real transfer, we propose a model-free deep reinforcement learning approach trained in simulation and then transferred to the robot without further fine-tuning. We therefore present a simulation environment that produces realistic normal forces, which we use to train continuous force control policies. An evaluation in which we compare against a baseline and perform an ablation study shows that our approach outperforms the hand-modeled baseline and that our proposed inductive bias and domain randomization facilitate sim-to-real transfer. Code, models, and supplementary videos are available on https://sites.google.com/view/rl-force-ctrl

==> sections/conclusion.tex <==
\section{CONCLUSION}

In this work, we presented a DRL method to train grasp force controllers for 2-DoF grippers in simulation and subsequently transfer them to the real robot without fine-tuning.
We proposed a novel simulation environment that generates realistic grasp forces, which we used to train our policies.
To strengthen the transfer performance, we proposed to use an inductive bias and domain randomization.
An extensive real-world evaluation has shown that our method can successfully grasp objects of highly varying stiffnesses while minimizing object movements during the grasp. 
Conclusively, our results show that continuous force control policies can be learned end-to-end is simulation and slightly outperform hand-modeled controllers on real robots.
An interesting direction for future work is the integration of grasp force control in more complex tasks for which DRL methods are used.

==> sections/environment.tex <==
\section{FORCE CONTROL SIMULATION}
\label{sec:env}

To train force control policies, we first modeled TIAGo's 2-DoF parallel jaw gripper in MuJoCo with one tactile sensor per finger and an object of variable softness.
The control frequency was set to \SI{25}{\Hz} to match that of a real TIAGo.

\begin{figure}[t!]
\centering
\includegraphics[width=0.9\linewidth]{images/gripper_scheme.pdf}
\caption{Schematic overview of the grasping scenario with the world frame $W$ and the object frame $O$. $w_o$ is the object width, $d_p$ its maximum deformation, and $o_y$ its position on the world's $y$-axis.}
\label{fig:gripper_scheme} 
\vspace{-0.4cm}
\end{figure}

\subsection{Grasping Scenario}

\begin{figure*}[t!]
\hfill
\begin{subfigure}[b]{0.325\linewidth}
   \includegraphics[width=1\linewidth]{images/act_var.pdf}
   \caption{Variation of $b_2$, changing finger velocity}
   \label{fig:act_var} 
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.325\linewidth}
   \includegraphics[width=1\linewidth]{images/solimp_var.pdf}
   \caption{Variation of $\rho$, changing \dfdq}
   \label{fig:solimp_var} 
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.325\linewidth}
   \includegraphics[width=1\linewidth]{images/fscale_var.pdf}
   \caption{Variation of $\kappa$, changing \dfdq and $f(T)$}
   \label{fig:fscale_var} 
\end{subfigure}
\hfill
\caption{\small Results from the real-world grasping trials conducted to determine realistic simulation parameters. Each plot shows the effect of varying one of the parameters discussed in \Secref{sec:env}, where $b_2$ changes actuator behavior and $\kappa$ affects the forces by changing $\rho$ and $\fscale$.}
\vspace{-0.4cm}
\end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{images/stiff_comp.pdf}
\caption{\small Comparison of final forces $f(T)$ of Sponge and Wood for grasps with different \dqdes. The regression slopes are 278 and 330. }
\label{fig:stiffness_plot} 
\vspace{-0.4cm}
\end{figure}


A schematic overview of the grasping scenario we consider is shown in \figref{fig:gripper_scheme}, which details all parameters needed to define it.
The gripper is depicted in its fully open state ($q_i = q_i^\text{max} = 0.045$), with an object located between the fingers somewhere on the grasping axis.
$W$ and $O$ refer to the world and object frames, where $W$ is considered fixed w.r.t. the gripper base and centered between the fingertips.
If the offset $\oy$ is non-zero, the symmetric object is displaced w.r.t. to this center, causing one fingertip to touch it earlier than the other.
The object width is defined by \wo and the maximum penetration depth (or object deformation) is given by \pdep.
Softer objects can be deformed more heavily and thus have larger values for \pdep.
As the controller should learn to maintain the object position during grasping, we sample \oy during episode initialization, thus exposing the learner to different object-gripper alignments.
\wo is also varied, such that the policy does not implicitly assume all objects to be of equal width.
The following three constraints are imposed on the sampling of the parameters:
\begin{align}
|\oy| + r_o &< \qmax \label{eq:const_qmax} \\
r_o -\pdep  &> |\oy| \label{eq:const_oy} \\
\pdep &< r_o \label{eq:const_wodp}
\end{align}
where $r_o = \frac{1}{2}\wo$ is the object radius.
\Eqref{eq:const_qmax} ensures that the object doesn't initially collide with a finger and \eqref{eq:const_oy} that the fingers can fully close up to the maximum penetration without dislocating the object core.
Finally, \eqref{eq:const_wodp} ensures that the object deformation is limited by the object radius.

The maximum object deformation \pdep cannot be defined directly in MuJoCo, but is determined by the softness of its contact constraints and the applied force.
To determine a realistic value, we calibrated the simulation against the real world by comparing the maximal deformation achieved during a power grasp, i.e. applying maximum force for a target position $\qdes_i = 0$.
% Choosing the correct softness value is more involved, however, as it requires real-life experiments to determine the range of realistic values.
%To determine \pdep, we simply executed a power grasp (closing with maximum force by setting the desired joint positions $\qdes_i = 0$) after determining said range.

\subsection{Actuator Behavior}

First, we tune the actuator parameters within MuJoCo to match the real robot behavior.
TIAGo uses position controllers, and to keep control signals identical, we opt to use them in the simulation as well.
While MuJoCo receives desired positions as control signals, our environment takes the desired position \emph{deltas} instead, converts them to desired positions internally, and forwards them to the simulation.
The joints are thus controlled by
\begin{align}
    \qdes_i = q_i + u_i
\end{align}
at each simulation step $t$, where $u_i = \dqdes_i$ is the control signal the policy or a user passes to the environment.
Using position deltas instead of positions directly has several advantages for the learning process.
First, the action space is symmetric and centered around zero with known bounds, making it easy to normalize while satisfying assumptions some RL algorithms make about the action space.
Second, by constraining the control signals with $|u_i| \leq \dqmax$, the maximum joint velocity is bounded and prevents the policy from executing erratic and potentially dangerous movements.
Choosing \dqmax is straightforward by executing different gripper closing trials with increasing values for \dqmax and setting it to the value resulting in the highest velocity within safety limits.
In all experiments, we set $\dqmax = 0.003$.

After defining the control, we tuned the actuators in MuJoCo to match the behavior of TIAGo. 
First, \textit{gainprm} and \textit{ctrlrange} were set to $[0.0, 0.045]$ and $[100, 0, 0]$ to mimic the real joint actuation range $[0, 0.045]$, which reflects the desired finger position in centimeters (see \figref{fig:gripper_scheme}).
Then, the third parameter of \textit{biasprm}, $b_2$, was tuned to match the finger's closing velocity and acceleration.
In order to find a range of realistic values for $b_2$, we executed power grasps with the real robot and in simulation, and then manually tuned $b_2$ until the joint trajectories matched.
We found $b_2 = -9$ to mirror the real behavior best, and $b_2 \in [-13, -6]$ to result in realistic actuator behavior for our domain randomization, which is shown in \figref{fig:act_var}.

\subsection{Force \& Softness Modeling}

After identifying realistic actuator parameters, the contact forces need to be modeled to imitate real-world objects as well. 
In MuJoCo, the softness of contact constraints can be changed with the \textit{solimp} parameters, which allow more object penetration, resulting in different \dqdf.
We set  \textit{solimp}'s first parameters, $d_\text{min} = 0$ to allow constraints to be maximally soft and use its \textit{width} parameter, which we refer to as $\rho$, to vary the constraint softness for each trial.

In order to find a range of realistic values for $\rho$, we executed real-life grasping trials on a soft and a rigid object (Sponge and Wood from \figref{fig:objects}).
Then, we conducted the same experiment in simulation, compared \dfdq for both experiments and tuned $\rho$ until the changes in force w.r.t. the joint position matched the real world trials for both objects.
\Figref{fig:solimp_var} shows force trajectories for the determined interval $\rho \in [0.003, 0.01]$.

Note, that changing the constraint stiffness $\rho$ results in different \dfdq, but not in different final forces.
In reality however, the force exerted on a stiff object is higher than one exerted on a soft object for the same \dqdes.
To also model this behavior, we introduced a force scaling factor \fscale, such that stiffer objects generate higher forces more quickly, and softer objects slower.
We conducted another set of grasping trials on the same objects, where a small, constant \dqdes was commanded to both fingers, and after the object was being held for a short amount of time, the final force $f(T)$ was noted.
The gripper was then opened again, \dqdes increased by $3 \times 10^{-4}$ and the experiment repeated until \dqdes = \dqmax.
Then, we repeated the same experiment in simulation, and  regressed $f(T)$ to \dqdes for both experiments.
The experiment data from the robot trials are shown in \figref{fig:stiffness_plot}.
\fscale is then the factor needed to match the regression slope of the simulation experiments with that of the real robot.
This way, we determined $\fscale \in [0.5, 5]$.

Lastly, to determine both values for $\rho$ and \fscale, we define a unified stiffness factor $\kappa \in [0, 1]$ which we use to interpolate within their respective intervals.
This way, we prevent unrealistic object configurations, e.g.\ a soft object with a high \fscale.




==> sections/experiments.tex <==
\section{EXPERIMENTAL EVALUATION}

For the experiments, we use Proximal Policy Optimization (PPO) \cite{schulmanProximalPolicyOptimization2017} to train the grasping policies.
We first evaluate our proposed method in simulation, and then apply the policies to the real robot and compare them in terms of force reward and object movements.

\subsection{Simulation experiments}
\begin{table*}[t]
\begin{center}
\caption{\small Real-world experimental results for six household testing objects. Our method \polib performs strongest of all models in terms of reward, and minimized object movements as efficiently as the baseline controller. The other models consistently performed worse.} 
\label{table:real_eval}
\scriptsize
\scalebox{1.0}{
\begin{tabular}{l|c||c|c|c|c|c|c||c}

Model & Metric & Rubber Mat & Sponge & Spray & Pringles & Wood & Mug & Average\\
\hline
\hline

\multirow{2}{*}{Baseline} & 
    \multirow{2}{*}{\shortstack{ Reward \\ Obj.Mov. }} &
    \multirow{2}{*}{\shortstack{ $92 \pm 15$  \\ $1.6 \pm 0.8$   }} & 
    \multirow{2}{*}{\shortstack{ $96 \pm 14$  \\ $\textbf{3.1} \pm \textbf{2.1}$   }} & 
    \multirow{2}{*}{\shortstack{ $\textbf{114} \pm \textbf{5}$  \\ $1.9 \pm 0.6$   }} & 
    \multirow{2}{*}{\shortstack{ $\textbf{118} \pm \textbf{7}$  \\ $\textbf{0.9} \pm \textbf{0.4}$   }} & 
    \multirow{2}{*}{\shortstack{ $\textbf{108} \pm \textbf{7}$  \\ $1.0 \pm 0.9$   }} & 
    \multirow{2}{*}{\shortstack{ $115 \pm 10$  \\ -   }} &
    \multirow{2}{*}{\shortstack{ $107 \pm 10$  \\ $\textbf{1.7} \pm \textbf{0.9}$   }} \\
&&&&&&&&\\
\hline

\multirow{2}{*}{\polib} & 
    \multirow{2}{*}{\shortstack{ Reward \\ Obj.Mov. }} &
    \multirow{2}{*}{\shortstack{ $\textbf{96} \pm \textbf{15}$  \\ $\textbf{1.5} \pm \textbf{0.8}$   }} & 
    \multirow{2}{*}{\shortstack{ $\textbf{103} \pm \textbf{7}$  \\ $3.2 \pm 1.4$   }} & 
    \multirow{2}{*}{\shortstack{ $109 \pm 17$  \\ $\textbf{1.8} \pm \textbf{0.8}$   }} & 
    \multirow{2}{*}{\shortstack{ $115 \pm 16$  \\ $1.2 \pm 0.6$   }} & 
    \multirow{2}{*}{\shortstack{ $105 \pm 15$  \\ $\textbf{0.7} \pm \textbf{0.7}$   }} & 
    \multirow{2}{*}{\shortstack{ $\textbf{120} \pm \textbf{10}$  \\ -   }} &
    \multirow{2}{*}{\shortstack{ $\textbf{109} \pm \textbf{13}$  \\ $\textbf{1.7} \pm \textbf{0.9}$  }} \\
&&&&&&&&\\
\hline

\multirow{2}{*}{\polnoib} & 
    \multirow{2}{*}{\shortstack{ Reward \\ Obj.Mov. }} &
    \multirow{2}{*}{\shortstack{ $77 \pm 10$  \\ $2.8 \pm 1.4$   }} & 
    \multirow{2}{*}{\shortstack{ $74 \pm 26$  \\ $4.0 \pm 0.9$   }} & 
    \multirow{2}{*}{\shortstack{ $88 \pm 33$  \\ $2.4 \pm 0.7$   }} & 
    \multirow{2}{*}{\shortstack{ $98 \pm 34$  \\ $1.9 \pm 0.6$   }} & 
    \multirow{2}{*}{\shortstack{ $101 \pm 16$  \\ $1.7 \pm 0.4$   }} & 
    \multirow{2}{*}{\shortstack{ $106 \pm 17$  \\ -   }} &
    \multirow{2}{*}{\shortstack{ $89 \pm 23$  \\ $2.6 \pm 0.8$    }} \\
&&&&&&&&\\
\hline

\multirow{2}{*}{\polnorand} & 
    \multirow{2}{*}{\shortstack{ Reward \\ Obj.Mov. }} &
    \multirow{2}{*}{\shortstack{ $82 \pm 12$  \\ $2.6 \pm 1.6$   }} & 
    \multirow{2}{*}{\shortstack{ $97 \pm 15$  \\ $3.6 \pm 1.3$   }} & 
    \multirow{2}{*}{\shortstack{ $57 \pm 37$  \\ $2.6 \pm 0.9$   }} & 
    \multirow{2}{*}{\shortstack{ $53 \pm 39$  \\ $1.7 \pm 0.7$   }} & 
    \multirow{2}{*}{\shortstack{ $49 \pm 33$  \\ $1.8 \pm 0.9$   }} & 
    \multirow{2}{*}{\shortstack{ $40 \pm 41$  \\ -   }} &
    \multirow{2}{*}{\shortstack{ $66 \pm 30$  \\ $2.5 \pm 1.1$    }} \\
&&&&&&&&\\
\hline 
\end{tabular}}
\end{center}
\vspace{-0.4cm}
\end{table*}

We run training for a total of 4M steps with an episode length of 150 steps and anneal the aforementioned parameters until $s_\text{end} = 1.5\text{M}$, whose initial and final values are given in \tabref{tab:params}.
In the beginning of each episode, all randomization parameters are sampled anew.
Our network consists of two fully connected layers with 50 neurons each and ReLu activations.
The output layer has two neurons, one per each finger's desired position delta.
We found a learning rate of $6 \times 10^{-4}$ to perform best, and the remaining parameters are set to their default values from stable-baselines3~\cite{sb3}.
We store model weights each time it surpasses the prior best reward averaged over 30 episodes.

We compare our policy with inductive bias \polib to a Python implementation of the grasp force controller presented in~\cite{lachBioInspiredGraspingController2022}, a policy \polnoib trained without the inductive bias, and a policy \polnorand trained with neither inductive bias nor domain randomization.
We evaluated both models on 11 stiffness values $\kappa$ (spaced out evenly in $[0,1]$, including interval borders) for 200 simulation trials each, summing up to 2200 trials per model and 8800 trials in total.
Note, that during these trials all other environment parameters except $\kappa$ were randomly sampled for each trial.
\Figref{fig:sim_eval} shows a box plot of cumulative episode rewards for each model at each value for $\kappa$.

While the baseline and both models with domain randomization perform well on all stiffness values, \polnorand shows much poorer performance overall.
Even though \polnorand was trained with a fixed $\kappa = 0.5$, it did not perform well for that value.
This is likely due to $b_2$ being varied in the evaluation while it was kept fix in the training of \polnorand.
Hence, it shows poor transfer performance to environments outside its training distribution.
The high performance of \polnoib indicates, that the reward term in \eqref{eq:rew2} is sufficient to learn the stopping behavior in simulation.
These results show that our method is capable of reliably learning grasp force control while minimizing object movements in simulation.

\begin{table}
\begin{center}
\captionof{table}{\small Annealed parameters with their initial and final values.} 
\label{tab:params}
\scriptsize
\begin{tabular}{l|cc}
     & Initial & Final  \\
\hline
\hline
$\alpha_2$  & 0 & 1.0  \\
\oydotmax   & $2 \times 10^{-4}$ & $5 \times 10^{-5}$  \\
\WO         & $[0.020, 0.025]$ & $[0.015, 0.035]$  \\
\OY         & $[0.0, 0.0]$ & $[-0.040, 0.040]$  \\
\hline
\end{tabular}
\end{center}
\vspace{-0.4cm}
\end{table}

\subsection{Real-World Evaluation}

To assess whether our policies are general enough to be transferred to the real robot, we evaluate them on TIAGo using six test objects of varying stiffness.
We perform 20 grasping trials per object and method, yielding $6 \times 4 \times 20 = 480$ trials in total.
In each trial, the object is offset to one finger, in half of the trials it is placed closer to the left finger, in the other half closer to the right.
During the grasp, the object is placed on millimeter paper, allowing us to measure its movements during the grasp.
Then, the model is commanded to perform a grasp, and after 6 seconds (150 steps at \SI{25}{\Hz}) the gripper is automatically opened again.
After the reward is computed and the traveled distance measured, the process repeats.
Note, that the reward is not directly comparable to the simulation results, as it only includes the force reward.
The object movement penalty would require measuring the object velocity at each time step: since this information is not available to us, we opted to measure the total object displacement after each trial instead.

\Tabref{table:real_eval} shows the results of the real-world evaluation.
\polib shows the strongest overall performance with an average reward of 109, while the baseline achieved a slightly lower average reward of 107.
Our experiments show that the inductive bias indeed facilitates sim-to-real performance, as evident by the lower average reward and higher object movements of \polnoib.
Furthermore, the (mostly) poor performance of \polnorand shows that domain randomization is a vital ingredient for both, generalization over different objects and sim-to-real transfer.
\polnorand was able to perform well on rather soft objects however, likely because they behave similarly to the simulation object configuration it trained on with $\kappa=0.5$, and our default choice for $b_2$ closely mirrors the robot behavior.
Note, that all models exhibit slightly worse performance in terms of object movements for the Sponge as compared to other objects.
This is due the Sponge being so light, that the sensors sometimes fail to detect first contact, a phenomenon also reported in \cite{lachBioInspiredGraspingController2022}.

The evaluation clearly shows that domain randomization is crucial for successful zero-shot policy transfer, and that domain knowledge in the form of inductive biases further facilitates the transfer.
Without any domain randomization, policies will overfit to their narrow training distribution and fail to generalize.
Our proposed simulation environment has shown to generate realistic forces, such that the transfer was possible for continuous control policies.
Videos of all models can be found in the supplementary material.

==> sections/introduction.tex <==
\section{INTRODUCTION}
%Proposal for introduction. Change/add/remove what you want
For humans and robots alike, tactile information is crucial in manipulation tasks involving environment contacts, visual occlusions, or both.
As a consequence, efforts of the robotics community to include this essential sensor modality have heavily increased over the past years \cite{bartolozziRobotsSenseTouch2016, dahiyaRoboticTactileSensing2013, dahiyaTactileSensingHumans2010}.
Prominent examples of tasks where tactile-based methods have shown successful include force control\cite{romano2011human, lachBioInspiredGraspingController2022}, object pushing\cite{churchTactileSimtoRealPolicy, pengSimtoRealTransferRobotic2018, linTactileGymSimtoreal2022}, and opening doors \cite{kalakrishnanLearningForceControl,kangVersatileDoorOpening2023}.

The application domain of tactile sensors is as diverse as the sensing principles within the field.
Complex sensors are commonly used in more challenging, high-level tasks such as surface following or edge prediction, which often involve deep learning methods\cite{zhangRoboticCurvedSurface2020, dingSimtoRealTransferOptical2020, dingSimtoRealTransferRobotic2021, pengSimtoRealTransferRobotic2018, lachPlacingTouchingEmpirical2023} or dexterous manipulation tasks\cite{maoLearningFinePinchGrasp2023, melnikUsingTactileSensing2021}.
Low-level tasks like force control are commonly modeled by hand\cite{romano2011human, tahara2010dynamic, li2012towards, lachBioInspiredGraspingController2022}, while those that use learning either rely on classical learning methods, do not investigate sim-to-real transfer, or both \cite{kalakrishnanLearningForceControl, dengGraspingForceControl2020, merzicLeveragingContactForces2018a, perrusquiaPositionForceControl2019, luoReinforcementLearningVariable2019}.
In contrast, this paper presents a deep reinforcement learning (DRL) approach for the low-level task of grasp force control for parallel-jaw grippers with two degrees of freedom (DoFs).
Similar to \cite{lachBioInspiredGraspingController2022}, our controller has two distinct control objectives to ensure safe object grasping and holding: I) reaching and maintaining a given goal force, and II) minimizing object movements while closing and holding the object.
Using normal forces measured at the fingertips, we train a continuous control policy in simulation and subsequently transfer it to the real robot.
We propose using to employ commonly used methods, an inductive bias\cite{zambaldiDEEPREINFORCEMENTLEARNING2019, hesselInductiveBiasesDeep2019} and domain randomization\cite{zhaoSimtoRealTransferDeep2020, juTransferringPolicyDeep2022}, to facilitate zero-shot sim-to-real transfer.
In an extensive real-world evaluation we compare our approach with a hand-modeled baseline from \cite{lachBioInspiredGraspingController2022} and conduct an ablation study over the two proposed methods.
We find the inductive bias to improve sim-to-real transfer and domain randomization to be vital for policies to generalize across real-world objects.

% In this work, we present a grasp force controller for 2-Degrees of Freedom (DoF) grippers that is learned in simulation using DRL, and subsequently transferred to the real robot in a zero-shot fashion (i.e.\ without further policy refinement on the robot).

\begin{figure}[t]
\hfill
\begin{subfigure}[b]{0.45\linewidth}
   \includegraphics[width=1\linewidth]{images/tape_grasp.jpg}
   \caption{Exemplary real-life grasp}
   \label{fig:real_grasp} 
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.51\linewidth}
   \includegraphics[width=1\linewidth]{images/object_wo02_oy0.png}
   \caption{Simulated scenario}
   \label{fig:sim_grasp} 
\end{subfigure}
\hfill
\caption{Safely holding an easily deformable object in real-life (a) vs. the simulation environment the policies are trained on (b).} \label{fig:introFig}
\vspace{-0.6cm}
\end{figure}

In the following, we propose a simulation environment based on MuJoCo\cite{todorovMuJoCoPhysicsEngine2012a}, where we tuned contact model parameters to match a few real-world samples.
Then, we detail our learning process based on deep reinforcement learning, where we apply domain randomization and introduce an inductive bias to learn policies for subsequent sim-to-real transfer.
Lastly, we compare our policy to a hand-modeled force controller~\cite{lachBioInspiredGraspingController2022} and perform an ablation study on some model choices. 
Our main contributions are: i)
a training procedure based on reinforcement learning that generalizes zero-shot to the real robot, ii) a novel simulation environment for 2-DoF grippers with realistic fingertip forces, and iii) open-sourcing the code for the environment, all methods and their evaluation and CAD models of the sensorized gripper.
To the best of our knowledge, this is the first paper proposing a tactile-based continuous grasp force controller learned with DRL which was transferred to the real robot without further refinement.




==> sections/related_work.tex <==
\section{RELATED WORK}

\noindent\textbf{Grasp Force Control} 
In their review of human grasping, Johansson and Flanagan~\cite{johansson2009coding} highlight the importance of tactile sensations, and divide the human grasping sequence into distinct phases, where tactile events often mark phase transitions.
Other experimental works have supported their findings~\cite{Sundaram2019}, and many contributions from robotics have adapted this human-inspired approach~\cite{romano2011human, lachBioInspiredGraspingController2022, Hsiao2010, Patel2018}.
Romano et al.~\cite{romano2011human} closely follow the phase distinctions from \cite{johansson2009coding} while modeling their force controller for the PR2 robot, but assume the fingers to be equidistant to the object while grasping.
Hsiao et al. \cite{Hsiao2010} also proposed a force controller for the PR2 that was integrated into its grasping pipeline\cite{Ciocarlie2014}, but without the assumption of equidistant finger-object placement.
These works hand-model controllers for grippers with a single degree of freedom, while our work relies on a learning approach that works for 2-DoF grippers.

Other works have proposed classical force controllers for end-effectors with two or more degrees of freedom.
The authors in \cite{Patel2018} designed a custom sensor that measures forces and proximity to ensure safe object grasps for their 2-DoF gripper.
The studies \cite{Su2015} and \cite{montano2018} use two fingers of a multi-fingered hand to perform force control, where the former detects slippage and regulates the grasp force accordingly, and the latter optimizes the fingertip positions based on force-closure constraints.
Another body of works has presented force controllers for more complex, multi-fingered hands\cite{tahara2010dynamic, li2012towards, Hang2016, Deng2020}.
As opposed to our work, these studies focus on more complex end-effectors while not employing DRL methods.

Learning grasp force control has also become popular in recent years. 
In \cite{merzicLeveragingContactForces2018a}, the authors learn a grasping policy that controls forces on rigid objects in simulation, while others focus on increasing grasp success using tactile feedback \cite{Wu2019}.
Others have learned to control grasping forces for more complex tasks like door opening\cite{kangVersatileDoorOpening2023}, high-precision assembly tasks\cite{luoReinforcementLearningVariable2019}, or surface tracking\cite{zhangRoboticCurvedSurface2020}.
The work of \cite{kalakrishnanLearningForceControl} uses classical RL learn force control policies, \cite{dengGraspingForceControl2020} combines deep learning with Gaussian Mixture Models, and \cite{perrusquiaPositionForceControl2019} use RL and admittance control to control forces in unknown environments.
Although these works learn force control behaviors, none of them investigate the potential of learning them in simulation and transferring them to the real robot afterwards.

\noindent\textbf{Sim-to-real transfer}
Sim-to-real transfer is widely used in robotics \cite{zhaoSimtoRealTransferDeep2020, juTransferringPolicyDeep2022} to avoid the time-consuming and labor-intensive task of real-world data collection.
For policies without tactile information, a commonly used approach is domain randomization \cite{zhaoSimtoRealTransferDeep2020, juTransferringPolicyDeep2022} of the visual input \cite{jamesSimToRealSimToSimDataEfficient2019, akkaya2019solving}.
In the domain of optical tactile sensors, \cite{churchTactileSimtoRealPolicy, linTactileGymSimtoreal2022} presented Tactile Gym, a simulation environment containing the TacTip\cite{ward-cherrierTacTipFamilySoft2018}, DIGIT\cite{lambetaDIGITNovelDesign2020} and DigiTac\cite{leporaDigiTacDIGITTacTipHybrid2022} sensors, and propose a domain adaptation approach by training adversarial networks on real-world data to generate tactile feedback in simulation. 
% \cite{yangSimtoRealModelBasedModelFree2023} showed sim-to-real transfer using this environment for model-based and model-free approaches for object pushing.
Later studies \cite{yangSimtoRealModelBasedModelFree2023, linBiTouchBimanualTactile2023} have reported successful sim-to-real transfer using Tactile Gym on various tasks, while others proposed simulators for the GelSlim \cite{donlonGelSlimHighResolutionCompact2018, xuEndtoEndDifferentiableFramework2021} and GelSight \cite{yuanGelSightHighResolutionRobot2017, chenBidirectionalSimtoRealTransfer2022, siGraspStabilityPrediction2022} sensors.
In contrast to these studies, we focus on low-level force control tasks which solely require force measurements as inputs.
Peng et al. \cite{pengSimtoRealTransferRobotic2018} chose to learn and transfer an object pushing policy for the Fetch robot.
Their work relies heavily on domain randomization and the authors argue that the robustness of the transferred policies was greatly increased.
Ding et al. \cite{dingSimtoRealTransferOptical2020} have proposed a Unity-based simulation of the TacTip sensor for edge prediction and have achieved sim-to-real transfer through domain randomization.
In a later work, Ding et al. \cite{dingSimtoRealTransferRobotic2021} use MuJoCo to simulate a selfmade tactile sensor array to open up a cabin door.
They again employ domain randomization for transferring the policy, but note that they binarized the sensor readings due to low sensitivity of the built-in MuJoCo touch sensor.
Although the authors in \cite{akkaya2019solving} also mention potential lack of realism in simulated continuous force measurements, we find that continuous force control policies can indeed be learned in MuJoCo and then be successfully transferred to the real world without fine-tuning.

Approaches based on Finite Element Methods (FEM), are capable of generating accurate simulation data of complex tactile sensors.
In \cite{narangSimtoRealRoboticTactile2021, narangInterpretingPredictingTactile2021}, the authors use FEM to estimate deformations of a BioTac\cite{fishelSensingTactileMicrovibrations2012} sensor and synthesize simulated data by learning a latent space representation.
Other papers have applied FEM to their custom-built soft tactile sensors \cite{sferrazzaDesignMotivationEvaluation2019, sferrazzaLearningSenseTouch2020, sferrazzaSimtorealHighresolutionOptical2021}.
Due to their high computational cost, FEM are typically not well-suited for data-driven approaches like DRL which we use, unless some simplifying assumptions can be made \cite{biZeroShotSimtoRealTransfer2021}.

==> sections/rl_task.tex <==
\section{LEARNING METHODS}

As the task of force control is a sequential decision-making problem, we can model it as a Markov Decision Process (MDP), allowing us to solve the problem using RL algorithms.
We follow the classical formulation of an MDP, which is defined as a tuple $\mathcal{M} = \langle \mathcal{S}, \mathcal{A}, P, r, \gamma, \iota\rangle$, 
with the state space $\mathcal{S}$, the action space $\mathcal{A}$, the transition kernel $P: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow \mathbb{R}^+$,  the reward function $r: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$, the discount factor $\gamma$, and the initial state distribution $\iota: \mathcal{S} \rightarrow \mathbb{R}^+$.
% with the state space $\mathcal{S}$, the action space $\mathcal{A}$, the state transition function 
%  $P(s_{t+1} | a_t, s_t)$, which is defined as a probability density over all states, indicating the probability of transitioning into $s_{t+1}$ from $s_t$ by taking action $a_t$, the reward function $r(s_t, a_t)$ gives the reward for taking the $a_t$ in state $s_t$.
The objective of Reinforcement learning algorithms is to find the optimal policy $\pi^*$ maximizing the expected discounted return $\mathcal{J}(\pi) = \mathbb{E}_{\tau\sim P, \pi, \iota}\left[\sum_{t=0}^{T} \gamma^t r(s_t,a_t)\right]$, where $\tau$ is a trajectory composed of a sequence of states and actions generated by executing the policy $\pi$ in the MDP.
% While the state transtition function is implicitly defined by the simulation environment, the rest of the tuple has yet to be defined.

\subsection{Observation Space}

The agent receives the following observation at each time step $t$:
\begin{gather}
o(t)
= \begin{pmatrix} 
% \begin{align}
q_i(t)\\
f_i(t) \\
\df_i(t) \\
a_i(t-1) \\
h_i(t) \\
% \end{align}
\end{pmatrix} 
\end{gather}
where subscript $i$ indicates that the observation is given for all joints $i$, $\df_i = \fgoal - f_i$  refers to the difference of the current force to the goal force, $a_i$ the last action taken by the agent (with $a_i(0) = [0,0]$) and $h_i$ being the \textit{had\_contact} flag.
The flag is defined as:
\begin{align}
  c_i(t) &= \begin{cases} 1 & \text{if}\,\, f_i(t) > f_\theta\\
    0 & \text{otherwise}
  \end{cases}\\
  h_i(t) &= c_i(t) \lor h_i(t-1)
\end{align}
where $c_i(t)$ indicates whether a finger is considered to be in contact with the object at time $t$ by comparing the current force to a noise threshold $f_\theta$, and $h_i(0) = 0$.
$h_i$ is 1 once $c_i$ was 1 before within the episode, even if the finger lost contact again ($c_i = 0$).
We provide this flag to avoid having a recurrent policy (since they can be difficult to train) or a long history of observations.
We add guassian noise to the joint position and fingertip force with $\sigma_q = 0.000027$ and $\sigma_f = 0.013$ and stack the observation $k=3$ times for the policy to have access to a short history of position and force deltas, so that it can estimate the object stiffness.

\subsection{Action Space}

% \begin{align}
% \ACT 
% = \begin{pmatrix} a_\text{left}   \\ a_\text{right}   \end{pmatrix} 
% = \begin{pmatrix} u_\text{left}   \\ u_\text{right}   \end{pmatrix}
% = \begin{pmatrix} \dq_\text{left} \\ \dq_\text{right} \end{pmatrix}
% \end{align}

The action space is simply a two-vector with one desired position per finger $(a_\text{left}, a_\text{right})^T$, where $a_i = \dqdes_i$ refers to an individual action for joint $i$.
Each $a_i$ is first clipped to lie within $[-1, 1]$ and then multiplied with \dqmax, effectively denormalizing $a_i$.

Additionally, we define a contact-state dependent inductive bias:
\begin{align}
    \phi_i = \begin{cases}
        \max(0.9, 1-\frac{|\df_i|}{\fgoal}) & \text{if} \,\, h_i = h_j = 1 \\
        0.1 & \text{if} \,\, h_i = 1 \land h_i \neq h_j \\
        1 & \text{else}
    \end{cases} 
\label{eq:indb}
\end{align}
that is multiplied with the individual actions at each time step, yielding $a_i' = \phi_i \, a_i$, which is then passed to the MuJoCo actuators.
It is inspired by the human grasping phases \cite{johansson2009coding} commonly used in other controllers \cite{romano2011human, lachBioInspiredGraspingController2022}, and  serves two purposes.
First,  it should aid the sim-to-real transfer of the policy by scaling down its control signal for an in-contact finger while the other is not yet in contact.
Second, it dampens the policy commands for in-contact states that are far from the goal as a safety measure.

\subsection{Reward Function}
\begin{figure}[t!]
\centering
\includegraphics[width=1\linewidth]{images/objects.jpg}
\caption{Evaluation objects: Rubber Mat, Sponge, Spray, Pringles, Wood and Mug. Ordered by increasing stiffness from left to right.}
\label{fig:objects} 
\vspace{-0.4cm}
\end{figure}

Our reward function mainly reflects the two controller objectives, and adds a third term for smoother control.
We propose the following individual reward terms:
\begin{align}
  \label{eq:rew1}
  \rforce &= 1 - \tanh\left (\ \sum_i |\Delta f_i|\right )\\ 
 \label{eq:rew2}
  \robj &=  \begin{cases} -1 & \text{if}\,\, \oydot > \oydotmax \\ 
                         0 & \text{otherwise}
             \end{cases} \\  
  \label{eq:rew3}
  \ract &= - \sum_i | a_i(t-1) - a_i(t) | 
\end{align}
The term \rforce reflects the first control objective in the reward function, namely to reach and maintain the target force.
$\tanh$ normalizes the force delta in $[0,1]$ and subtracting it from 1 yields the highest reward if $\sum\df_i = 0$.
\robj expresses the second controller objective as a reward function by penalizing object movements with a sparse reward of -1 upon constraint violation.
In equation \ref{eq:rew2},  \oydot refers to the current object velocity and \oydotmax to the object velocity threshold.
\oydot has shown to always be noisy during finger contact, hence we use the threshold $\oydotmax = 0.00005$.
The third reward term, \ract, penalizes high changes in policy actions at consecutive time steps to encourage a smooth control behavior.
Other, more involved procedures have been proposed before\cite{mysoreRegularizingActionPolicies2021}, but for our purposes this simple constraint has shown to be sufficient.
Finally, the total reward per time step is defined as
\begin{align}
    r = \alpha_1 \rforce + \alpha_2 \robj + \alpha_3 \ract
    \label{eq:totalr}
\end{align}

\subsection{Curriculum Learning}
\begin{figure}[t!]
\centering
\includegraphics[width=1\linewidth]{images/box.pdf}
\caption{Comparison of all four models for different $\kappa$ in simulation. Baseline and models with domain randomization show strong performance, while \polnorand performs poorly.}
\label{fig:sim_eval} 
\vspace{-0.4cm}
\end{figure}

Our reward function as it is given in \eqref{eq:totalr} poses a difficult problem for learning control policies:
during exploration it is highly likely that a random agent will push the object with one finger before it learns to precisely control the grasping force.
As a result, the policy will converge to local minima where it avoids contact with the object, since it will receive a large negative reward from \robj before being rewarded by \rforce.
We therefore employ a learning curriculum, a common approach to gradually increase the task complexity over the course of training by annealing certain environment parameters \cite{narvekarLearningCurriculumPolicies2018, narvekarCurriculumLearningReinforcement2020}.

The parameters controlling the likelihood of these high negative rewards are $\alpha_2$, the scaling factor for \robj, the range of possible object displacements \OY, the range of object radii \WO, and the object velocity threshold \oydotmax.
For the scalar parameter $\alpha_2$ and \oydotmax, a starting value and a final value are defined.
During training, the parameters are linearly interpolated at each time step from their initial value at $t=0$ until they reached their final value at $t=s_\text{end}$, where $s_\text{end}$ is a hyperparameter.
For the intervals \OY and \WO, the initial and final interval borders are given. 
During the annealing phase, both borders are also linearly interpolated from their respective initial to their final values.

